CHSEL: Producing Diverse Plausible Pose Estimates from Contact and Free Space Data

This paper proposes a novel method for estimating the set of plausible poses of a rigid object from a set of points with volumetric information, such as whether each point is in free space or on the surface of the object. In particular, we study how pose can be estimated from force and tactile data arising from contact. Using data derived from contact is challenging because it is inherently less information-dense than visual data, and thus the pose estimation problem is severely under-constrained when there are few contacts. Rather than attempting to estimate the true pose of the object, which is not tractable without a large number of contacts, we seek to estimate a plausible set of poses which obey the constraints imposed by the sensor data. Existing methods struggle to estimate this set because they are either designed for single pose estimates or require informative priors to be effective. Our approach to this problem, Constrained pose Hypothesis Set Elimination (CHSEL), has three key attributes: 1) It considers volumetric information, which allows us to account for known free space; 2) It uses a novel differentiable volumetric cost function to take advantage of powerful gradient-based optimization tools; and 3) It uses methods from the Quality Diversity (QD) optimization literature to produce a diverse set of high-quality poses. To our knowledge, QD methods have not been used previously for pose registration. We also show how to update our plausible pose estimates online as more data is gathered by the robot. Our experiments suggest that CHSEL shows large performance improvements over several baseline methods for both simulated and real-world data.

==> old_intro.tex <==
In robotic systems that manipulate objects such as for surgery~\cite{taylor2016medical}, and household use~\cite{billard2019trends}, a common intermediate step is to estimate the pose of the object with respect to the robot. This is often accomplished via point-set registration, a technique where points sampled from the object model are transformed and matched against observed points. Predominantly, the points on the object are perceived through vision [TODO: cite?], but in manipulation contexts it suffers from object transparency, occlusion (from other objects and the robot itself), and varying scene illumination. Traditional methods such as iterative closest point (ICP) struggles with these issues and has prompted many advances including:
\begin{itemize}
    \item registration using point features and semantics in addition to position~\cite{he2017iterative}~\cite{zhang2021new}
    \item relying on tactile sensors and local geometric features~\cite{villalonga2021tactile}
    \item explicitly treating known free-space points~\cite{haugo2020iterative}
\end{itemize}
[TODO: motivate plausible diversity (downstream uses)]
[TODO: introduce our method intuition and high level understanding]
Performance for all methods in general improve with increasing number of observed points, but tactile methods require making contact to collect data. Minimizing the number of contacts is ideal to minimize the chance of moving the object and as a measure of efficiency. As such, we evaluate methods on experiments that with sparse contacts.

Our method is agnostic to how the points are observed, but works well even with few points and when the points are imbalanced in terms of semantics, and so is suitable for contact-based tasks.

Especially towards the beginning of contact-based tasks, uncertainty in the object pose is high due to insufficient data, sensor noise, and inherent object symmetries. Characterizing this uncertainty is useful for object recognition, efficient exploration, and other downstream tasks [TODO: cite papers using these for downstream tasks such as sensor fusion, SLAM, and so on; consult SVGD-ICP for their citations]. Bayesian methods to capture the full distribution is intractable, and approximation techniques such as Markov Chain Monte Carlo (MCMC) and variational inference~\cite{maken2021stein} have been applied. [TODO: see their introduction and adopt parts of it] Empirically, we evaluate a Stein-variational optimization scheme as an alternative to quality diversity. In general, we found variational methods too dependent on informative priors

[TODO: no well-defined ground truth distribution and thus no good metrics for evaluating how good this distribution is approximated]

[TODO: method uses both point semantics and produces an uncertainty estimate]
